HINT: High-quality INPainting Transformer with Mask-Aware Encoding and Enhanced Attention

Existing image inpainting methods leverage convolution-based downsampling approaches to reduce spatial dimensions. This may result in information loss from corrupted images where the available information is inherently sparse, especially for the scenario of large missing regions. Recent advances in self-attention mechanisms within transformers have led to significant improvements in many computer vision tasks including inpainting. However, limited by the computational costs, existing methods cannot fully exploit the efficacy of long-range modelling capabilities of such models. In this paper, we propose an end-to-end High-quality INpainting Transformer, abbreviated as HINT, which consists of a novel mask-aware pixel-shuffle downsampling module (MPD) to preserve the visible information extracted from the corrupted image while maintaining the integrity of the information available for high-level inferences made within the model. Moreover, we propose a Spatially-activated Channel Attention Layer (SCAL), an efficient self-attention mechanism interpreting spatial awareness to model the corrupted image at multiple scales. To further enhance the effectiveness of SCAL, motivated by recent advanced in speech recognition, we introduce a sandwich structure that places feed-forward networks before and after the SCAL module. We demonstrate the superior performance of HINT compared to contemporary state-of-the-art models on four datasets, CelebA, CelebA-HQ, Places2, and Dunhuang.

==> Figures/long.tex <==
\begin{figure*}[t] \centering
    % \makebox[0.092\textwidth]{\footnotesize Input}
    % \makebox[0.092\textwidth]{\footnotesize DeepFill v1~\cite{yu2018generative}}
    % \makebox[0.092\textwidth]{\footnotesize DeepFill v2~\cite{yu2019free}}
    % \makebox[0.092\textwidth]{\footnotesize CTSDG~\cite{guo2021image}}
    % \makebox[0.092\textwidth]{\footnotesize LAMA~\cite{wan2021high}}
    % \makebox[0.092\textwidth]{\footnotesize MISF~\cite{li2022misf}}
    % \makebox[0.092\textwidth]{\footnotesize WNet~\cite{zhang2022w}}
    % \makebox[0.092\textwidth]{\footnotesize LDM~\cite{Rombach_2022_CVPR}}
    % \makebox[0.092\textwidth]{\footnotesize HINT (Ours)}
    % \makebox[0.092\textwidth]{\footnotesize GT}
    % \\
    \includegraphics[width=0.092\textwidth]{Images/long/Pls_1_input2.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Pls_1_df1.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Pls_1_df2.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Pls_1_CTSDG.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Pls_1_LAMA.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Pls_1_MISF.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Plc_1_WN.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Pls_1_LDM.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Pls_1_HINT.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Pls_1_gt.png}
    \\
    \includegraphics[width=0.092\textwidth]{Images/long/Pls_2_input.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Pls_2_df1.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Pls_2_df2.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Pls_2_CTSDG.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Pls_2_LAMA.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Pls_2_MISF.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Plc_2_WN.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Pls_2_LDM.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Pls_2_HINT.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Pls_2_gt.png}
    \\
    \includegraphics[width=0.092\textwidth]{Images/long/PLC_6_input.png}
    \includegraphics[width=0.092\textwidth]{Images/long/PLC_6_df1.png}
    \includegraphics[width=0.092\textwidth]{Images/long/PLC_6_df2.png}
    \includegraphics[width=0.092\textwidth]{Images/long/PLC_6_CTSDG.png}
    \includegraphics[width=0.092\textwidth]{Images/long/PLC_6_LAMA.png}
    \includegraphics[width=0.092\textwidth]{Images/long/PLC_6_MISF.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Plc_6_WN.png}
    \includegraphics[width=0.092\textwidth]{Images/long/PlC_6_LDM.png}
    \includegraphics[width=0.092\textwidth]{Images/long/PLC_6_HINT.png}
    \includegraphics[width=0.092\textwidth]{Images/long/PLC_6_gt.png}
    \\
    \includegraphics[width=0.092\textwidth]{Images/long/PLC_7_input.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Plc_7_df1.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Plc_7_df2.png}
    \includegraphics[width=0.092\textwidth]{Images/long/PLC_7_CTSDG.png}
    \includegraphics[width=0.092\textwidth]{Images/long/PLC_7_LAMA.png}
    \includegraphics[width=0.092\textwidth]{Images/long/PLC_7_MISF.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Plc_7_WN.png}
    \includegraphics[width=0.092\textwidth]{Images/long/PlC_7_LDM.png}
    \includegraphics[width=0.092\textwidth]{Images/long/PLC_7_HINT.png}
    \includegraphics[width=0.092\textwidth]{Images/long/PLC_7_gt.png}
    \\
    \vspace{-0.5em}
    \makebox[0.092\textwidth]{\footnotesize Input}
    \makebox[0.092\textwidth]{\footnotesize DeepFill v1~\cite{yu2018generative}}
    \makebox[0.092\textwidth]{\footnotesize DeepFill v2~\cite{yu2019free}}
    \makebox[0.092\textwidth]{\footnotesize CTSDG~\cite{guo2021image}}
    \makebox[0.092\textwidth]{\footnotesize LAMA~\cite{wan2021high}}
    \makebox[0.092\textwidth]{\footnotesize MISF~\cite{li2022misf}}
    \makebox[0.092\textwidth]{\footnotesize WNet~\cite{zhang2022w}}
    \makebox[0.092\textwidth]{\footnotesize LDM~\cite{Rombach_2022_CVPR}}
    \makebox[0.092\textwidth]{\footnotesize HINT (Ours)}
    \makebox[0.092\textwidth]{\footnotesize GT}
    \\
    \vspace{0.5em}
    % \includegraphics[width=0.092\textwidth]{Images/long/PLC_8_input.png}
    % \includegraphics[width=0.092\textwidth]{Images/long/PLC_8_CTSDG.png}
    % \includegraphics[width=0.092\textwidth]{Images/long/PLC_8_LAMA.png}
    % \includegraphics[width=0.092\textwidth]{Images/long/PLC_8_MISF.png}
    % \includegraphics[width=0.092\textwidth]{Images/long/PlC_8_LDM.png}
    % \includegraphics[width=0.092\textwidth]{Images/long/PLC_8_HINT.png}
    % \includegraphics[width=0.092\textwidth]{Images/long/PLC_8_gt.png}
    % \\
    % \makebox[0.092\textwidth]{\footnotesize Input}
    % \makebox[0.092\textwidth]{\footnotesize DeepFill v1~\cite{yu2018generative}}
    % \makebox[0.092\textwidth]{\footnotesize DeepFill v2~\cite{yu2019free}}
    % \makebox[0.092\textwidth]{\footnotesize WaveFill~\cite{yu2021wavefill}}
    % \makebox[0.092\textwidth]{\footnotesize LAMA~\cite{wan2021high}}
    % \makebox[0.092\textwidth]{\footnotesize WNet~\cite{zhang2022w}}
    % \makebox[0.092\textwidth]{\footnotesize MAT~\cite{li2022mat}}
    % \makebox[0.092\textwidth]{\footnotesize RePaint~\cite{Lugmayr_2022_CVPR}}
    % \makebox[0.092\textwidth]{\footnotesize HINT (Ours)}
    % \makebox[0.092\textwidth]{\footnotesize GT}
    % \\
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_1_input.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_1_df1.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_1_df2.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_1_WF.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_1_LAMA.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_1_WN.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_1_MAT.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_1_RePaint.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_1_HINT.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_1_gt.png}
    \\
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_2_input.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_2_df1.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_2_df2.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_2_WF.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_2_LAMA.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_2_WN.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_2_MAT.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_2_RePaint.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_2_HINT.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_2_gt.png}
    \\
    \includegraphics[width=0.092\textwidth]{Images/long/CLB_3_input.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_3_df1.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_3_df2.png}
    \includegraphics[width=0.092\textwidth]{Images/long/CLB_3_Wave.png}
    \includegraphics[width=0.092\textwidth]{Images/long/CLB_3_LAMA.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_3_WN.png}
    \includegraphics[width=0.092\textwidth]{Images/long/CLB_3_MAT.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_3_RP.png}
    \includegraphics[width=0.092\textwidth]{Images/long/CLB_3_HINT.png}
    \includegraphics[width=0.092\textwidth]{Images/long/CLB_3_gt.png}
    \\
    \includegraphics[width=0.092\textwidth]{Images/long/CLB_4_input.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_4_df1.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_4_df2.png}
    \includegraphics[width=0.092\textwidth]{Images/long/CLB_4_Wave.png}
    \includegraphics[width=0.092\textwidth]{Images/long/CLB_4_LAMA.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_4_WN.png}
    \includegraphics[width=0.092\textwidth]{Images/long/CLB_4_MAT.png}
    \includegraphics[width=0.092\textwidth]{Images/long/Clb_4_RP.png}
    \includegraphics[width=0.092\textwidth]{Images/long/CLB_4_HINT.png}
    \includegraphics[width=0.092\textwidth]{Images/long/CLB_4_gt.png}
    \\
    \vspace{-0.5em}
    \makebox[0.092\textwidth]{\footnotesize Input}
    \makebox[0.092\textwidth]{\footnotesize DeepFill v1~\cite{yu2018generative}}
    \makebox[0.092\textwidth]{\footnotesize DeepFill v2~\cite{yu2019free}}
    \makebox[0.092\textwidth]{\footnotesize WaveFill~\cite{yu2021wavefill}}
    \makebox[0.092\textwidth]{\footnotesize LAMA~\cite{wan2021high}}
    \makebox[0.092\textwidth]{\footnotesize WNet~\cite{zhang2022w}}
    \makebox[0.092\textwidth]{\footnotesize MAT~\cite{li2022mat}}
    \makebox[0.092\textwidth]{\footnotesize RePaint~\cite{Lugmayr_2022_CVPR}}
    \makebox[0.092\textwidth]{\footnotesize HINT (Ours)}
    \makebox[0.092\textwidth]{\footnotesize GT}
    \\
    % \includegraphics[width=0.092\textwidth]{Images/long/CLB_5_input.png}
    % \includegraphics[width=0.092\textwidth]{Images/long/CLB_5_Wave.png}
    % \includegraphics[width=0.092\textwidth]{Images/long/CLB_5_LAMA.png}
    % \includegraphics[width=0.092\textwidth]{Images/long/CLB_5_MAT.png}
    % \includegraphics[width=0.092\textwidth]{Images/long/Clb_5_RP.png}
    % \includegraphics[width=0.092\textwidth]{Images/long/CLB_5_HINT.png}
    % \includegraphics[width=0.092\textwidth]{Images/long/CLB_5_gt.png}
    % \\
    % \vspace{-0.7em}
    \caption{Comparisons with visualisations $(256 \times 256)$ showing that our results are more coherent in structure and sharper in texture and semantic details. The top two rows are from CelebA-HQ~\cite{karras2017progressive} and the bottom two rows are from Places2~\cite{zhou2017places}.} 
    % \vspace{-0.7em}
    \label{fig:comparison_CelebAHQ&Places2}
\end{figure*}


==> Figures/long_resolution.tex <==
\begin{figure}[t] \centering
    \makebox[0.23\textwidth]{\footnotesize Masked Input}
    \makebox[0.23\textwidth]{\footnotesize Ours}
    % \makebox[0.09\textwidth]{\footnotesize B (- Sandwich)}
    % \makebox[0.09\textwidth]{\footnotesize C (- SCAL) }
    % \makebox[0.09\textwidth]{\footnotesize D (Full)}
    % \makebox[0.09\textwidth]{\footnotesize GT}
    \\
    \includegraphics[width=0.23\textwidth]{Images/long_resolution/long_resolution1.png}
    \includegraphics[width=0.23\textwidth]{Images/long_resolution/long_resolution1_HINT.png}\\
    \includegraphics[width=0.23\textwidth]{Images/long_resolution/long_resolution2.png}
    \includegraphics[width=0.23\textwidth]{Images/long_resolution/long_resolution2_HINT.png}
    % \includegraphics[width=0.09\textwidth]{Images/Abl/Abl_1_woSandwich.png}
    % \includegraphics[width=0.09\textwidth]{Images/Abl/Abl_1_woSCAL.png}
    % \includegraphics[width=0.09\textwidth]{Images/Abl/Abl_1_HINT.png}
    % % \includegraphics[width=0.09\textwidth]{Images/Abl/Abl_1_gt.png}
    \\
    % \vspace{-0.7em}
    \caption{Two real-world examples with high-resolution.
    } 
    % \vspace{-1.4em}
    \label{fig:long_resolution}
\end{figure}

==> Tables/FID.tex <==
\begin{table}\centering
\captionsetup[table]{skip=4pt}
\caption{FID Comparison on CelebA-HQ.}
\label{tab:FID}
\scriptsize
\resizebox{0.50\textwidth}{!}{
    {
    \tabulinesep=0mm
    \begin{tabular}{*{5}{c}}
    \hline\hline
    Mask Ratios & WaveFill\cite{yu2021wavefill} & LAMA\cite{suvorov2022resolution} &  MAT\cite{li2022mat} & Ours\T\B\\
    \hline
    20\% & 6.0638 & 1.4309 & \underline{1.2428} & \textbf{1.1159} \T\\
    40\% & 8.3804 & 4.4295 & \textbf{3.4677} & \underline{4.3990} \\
    60\% & 13.0849 & 8.4538 & \textbf{5.7284} & \underline{7.5793}\B\\
    \hline\hline
    \end{tabular}
    }
    }
\end{table}
